Automated Attribution Graph Interpretation via Probe Prompting

Even though we know the precise computations that lead from a large language model (LLM) input to its output this computation remains very hard to interpret. One way to make it easier to understand this process is by creating a sparse computational graph that captures most of the model behavior with smallest number of computational nodes. Cross-layer transcoders (CLT) decompose the dense computations of the MLP but the resulting circuits still contain thousands of nodes even for short prompts. Existing automated interpretation methods label individual features from corpus activations, and it often happens that these labels are not validated by causal intervention. We introduce probe prompting, a transparent rule-based pipeline that groups the features of an attribution graph into concept-aligned supernodes from their responses on a small set of concept-targeted probe prompts, summarized as Cross-Prompt Activation Signatures (CPAS). Across four factual domains, on Gemma-2-2B with a public CLT dictionary and 45,596 entity-swap interventions, we find that the labeled supernodes have the predicted steering behavior in every one of them. Code, datasets, and an interactive demo are released anonymously as a reusable harness for calibrating supernode labels against causal interventions.

==> figures/swap_overview.tex <==
% Two single-column floats: matrix at top of the left column,
% 2x2 grid of representative interventions at top of the right column.
% Both [!t] and declared back-to-back so LaTeX fills the two top-of-column
% slots on the same page.

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/swap_matrix.pdf}
  \caption{Source $\to$ target swap matrix on the 50-state USA panel
    ($n{=}2{,}450$ pairs, hit-rate $69.8$\%). By default we steer on all
    three concept fields (state + capital + city); each cell additionally
    considers every smaller field subset and reports the winning
    configuration. The winner is the variant that hits the target capital
    (steered top-1 = target capital first-token); when several variants
    hit, we prefer the one that maximises the steered margin of the target
    logit over the next-best capital in the dataset.
    Cells are coloured by the winning field subset; the 3-field default
    wins only $13$\% of cells, the rest succeed with a strict subset. Grey cells: miss; black on
    the diagonal: pair not run.}
  \label{fig:swap-matrix}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=1\linewidth]{figures/swap_v2_in_mn.pdf}
  \caption{A representative entity-swap intervention on the USA panel:
    Indiana$\to$Minnesota, probed via ``the state containing Fort Wayne''.
    The top row shows the prompt and the pre/post-intervention prediction
    (\texttt{Indianapolis} $\to$ \texttt{St}, i.e.\ \texttt{Saint~Paul}). The
    middle row shows the labeled supernodes with ablation ($-2\times$) of the
    source state/capital nodes and amplification ($+20\times$) of the target
    state/capital nodes. The bottom row shows the next-token probability sweep
    at $M{=}0$ vs.\ $M{=}20$, with the target trajectory (\texttt{Saint}) rising
    at the steered position while the original (\texttt{Indianapolis}) collapses.}
  \label{fig:swap-examples}
\end{figure}


==> sections/experimental_design.tex <==
\section{Experimental Design}
\label{sec:expdesign}

\subsection{Domains and seed prompts}
\label{sec:expdesign:domains}
We evaluate on five domains spanning two-hop factual recall in different relational structures and answer geometries. Each domain has a fixed seed-prompt template with three semantic fields (input, intermediate, answer): USA (``capital of state containing $X$''; 50 entities, 2{,}450 non-identity swap pairs, answer-set size $K{=}50$), Books (``character $X$ from book by''; 16/240/25), Products (``product $X$ from company by''; 12/132/25), Paintings (``painting $X$ by painter''; 10/90/20), and Sounds (``sound $X$ from animal of color''; 6/30/6). The first four are the \emph{strong} domains used for cross-domain inference; Sounds has $12/30$ pairs sharing an answer and is reported separately as a directional negative (\cref{sec:results:negative}, \cref{sec:limitations}).

\subsection{Experimental matrix}
\label{sec:expdesign:matrix}
Each swap pair is run under: (a) labeled (3-field) baseline at $M{=}20$; (b) matched random control (3 replicates per pair); (c) field-additivity (7 variants per pair); (d) adaptive $M$-search on labeled and on the best field-add variant per missed pair. The total is \textbf{42{,}184 swap runs} across all conditions, domains, and $M$ values.

\subsection{Pre-registered evaluation choices}
\label{sec:expdesign:prereg}
Before running the sweep we fixed the evaluation protocol. The contrast set used by vsMax is the set of all other dataset answers in the same domain, and multi-token answers are resolved to their first subword so that Hit is a deterministic substring check. Intervention and measurement are explicitly decoupled: the intervention operates on supernodes tied to entity fields, while the Hit/vsMax readout is always taken on the answer field. Generation uses temperature $0.3$, a maximum of 10 new tokens, a frequency penalty of $2.0$, and a fixed seed; matched-control replicates are drawn with sha256-based seeding from the run seed and pair identifier. At the pair level we count a random-hit if any of the three matched-control replicates is a hit, so the random baseline is deliberately optimistic. Ranges, thresholds, and seeds were frozen prior to the 42{,}184-run sweep. Full details are in \cref{appx:pipeline}.


==> tables/T1_graph_vs_subgraph.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Pipeline output: compression with high coverage.} \emph{Repl.}\ = fraction of end-to-end influence routed via features; \emph{Comp.}\ = fraction of incoming edge influence explained. Concept-aligned subgraphs preserve Completeness ($0.83$ vs.\ $0.90$) while compressing $\sim$600$+$ raw features into 30--50 supernodes (Repl.\ drops $0.70\!\to\!0.54$). Descriptive only.}
\label{tab:graph-subgraph}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
\textbf{Prompt} & \textbf{G-Repl.} & \textbf{S-Repl.} & \textbf{G-Comp.} & \textbf{S-Comp.} \\
\midrule
Austin (Dallas)      & 0.72 & 0.57 & 0.90 & 0.83 \\
Oakland (swap)       & 0.70 & 0.57 & 0.90 & 0.83 \\
Michael Jordan       & 0.69 & 0.49 & 0.90 & 0.81 \\
Small opposite       & 0.73 & 0.62 & 0.91 & 0.86 \\
Muscle diaphragm     & 0.63 & 0.45 & 0.87 & 0.79 \\
\midrule
Mean                 & 0.70 & 0.54 & 0.90 & 0.83 \\
\bottomrule
\end{tabular}}
\end{table}




==> tables/T3_fieldadd.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Less-is-more (C2.1): smaller field subsets beat the all-three-field intervention.} Per-domain best subset vs.\ the all-3-field labeled baseline at $M{=}20$. In 4/5 domains the intermediate field carries the strongest signal; pairing it with the answer field yields a 9--33~pp gain. Per-variant tables in \cref{appx:fieldadd}.}
\label{tab:fieldadd}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrr}
\toprule
Domain & Best subset & Best\,Hit\% & All-3\,Hit\% & $\Delta$ \\
\midrule
USA       & state $+$ capital   & 38.8 & 24.7 & $+14.1$ \\
Books     & book $+$ author     & 37.1 &  3.8 & $+33.3$ \\
Products  & company $+$ founder & 24.2 & 15.2 &  $+9.0$ \\
Sounds    & sound $+$ animal    & 20.0 &  0.0 & $+20.0$ \\
Paintings & first\_name (1-fld) & ~6.7 &  3.3 &  $+3.4$ \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/T_domains.tex <==
\begin{table*}[t]
\centering
\small
\caption{\textbf{Five evaluation domains.} Each row gives the seed-prompt template, the three semantic fields (input / intermediate / answer), the answer-set size $K$, the number of entities and non-identity swap pairs, and the total run count across all conditions (labeled, matched-random $\times 3$, 7 field-additivity variants, adaptive-$M$ rescue). The four \emph{strong} domains (USA, Books, Products, Paintings) are used for cross-domain inference; \emph{Sounds} is reported separately as a directional negative (\cref{sec:results:negative}). Full per-condition counts in \cref{appx:specificity,appx:fieldadd,appx:msearch}.}
\label{tab:domains}
\begin{tabular}{llp{3.4cm}rrrr}
\toprule
Domain & Seed prompt template & Fields (in / int / ans) & $K$ & Entities & Pairs & Total runs \\
\midrule
USA       & ``capital of state containing $X$'' & city / state / capital       & 50 & 50 & 2{,}450 & $\approx$28{,}400 \\
Books     & ``character $X$ from book by''      & character / book / author    & 25 & 16 & 240     & $\approx$2{,}800  \\
Products  & ``product $X$ from company by''     & product / company / founder  & 25 & 12 & 132     & $\approx$1{,}700  \\
Paintings & ``painting $X$ by painter''          & painting / painter / first\_name & 20 & 10 & 90  & $\approx$1{,}200  \\
Sounds    & ``sound $X$ from animal of color''   & sound / animal / color       & 6  & 6  & 30      & $\approx$400      \\
\midrule
\multicolumn{6}{l}{\textbf{Total}} & \textbf{42{,}184} \\
\bottomrule
\end{tabular}
\end{table*}

